Non-Stochastic Control with Bandit Feedback

We study the problem of controlling a linear dynamical system with adversarial perturbations where the only feedback available to the controller is the scalar loss, and the loss function itself is unknown. For this problem, with either a known or unknown system, we give an efficient sublinear regret algorithm. The main algorithmic difficulty is the dependence of the loss on past controls. To overcome this issue, we propose an efficient algorithm for the general setting of bandit convex optimization for loss functions with memory, which may be of independent interest.

==> arxiv/7.1.ExpKnownDynamics-arxiv.tex <==


\subsection{Control with known dynamics}
We first evaluate our Algorithm \ref{alg2} (BPC) while comparing to GPC \citep{agarwal2019online}, as well as the baseline method Linear Quadratic Regulator (LQR) \citep{kalman1960general}. For both BPC and GPC we initialize $K$ to be the infinite-horizon LQR solution given dynamics $A$ and $B$ in all of the settings below in order to observe the improvement provided by the two perturbation controllers relative to the classical approach.

We consider four different loss functions: 
\begin{enumerate}
    \item $L_2^2$-norm: $c_t(x, u) = ||x||^2 +  ||u||^2$ (also known as \textit{quadratic cost}), 
    \item $L_1$-norm: $c_t(x, u) = ||x||_1 + ||u||_1$, 
    \item $L_{\infty}$-norm: $c_t(x, u) = ||x||_{\infty} + ||u||_{\infty}$,
    \item ReLU: $c_t(x, u) = ||\max(0, x)||_1 + ||\max(0, u)||_1$ (each max taken element-wise).
\end{enumerate}
We run the algorithms on two different linear dynamical system, the $n=2, m=1$ double integrator system defined by $A = \begin{bmatrix} 1 & 1 \\ 0 & 1 \end{bmatrix}$ and $B = \begin{bmatrix} 0  \\ 1\end{bmatrix}$, as well as one additional setting on a larger LDS with $n=5, m=3$ for sparse but non-trivial $A$ and $B$. We analyze the performance of our algorithms for the following 3 noise specifications.

\begin{enumerate}
    \item \textbf{Sanity check.} We run our algorithms with i.i.d Gaussian noise terms $w_t \sim \mathcal{N}(0, I)$. We see that decaying learning rates allow the GPC and BPC to converge to the LQR solution which is optimal for this setup.
    \item \textbf{Sinusoidal noise.} In this setup, we look at the sinusoidal $w_t = sin(t / (20\pi))$. In this correlated noise setting, the LQR policy is sub-optimal, and we see that both BPC and GPC outperform it.
    \item \textbf{Gaussian random walk.} In the Gaussian random walk setting, each noise term is distributed normally, with the previous noise term as its mean, i.e. $w_{t+1} = \mathcal{N}\left(w_t, \frac{1}{T}\right)$. Since $T = 1000$, we have approximately that $w_{t+1} - w_t \sim \mathcal{N} (0, 0.3^2)$.
\end{enumerate}


\begin{figure}[htp!]
    \centering
    \begin{tabular}{cc}
    \subfloat[Sanity check with fixed learning rate]{\includegraphics[width=0.24\textwidth] {Plots/PlotsKnown/no_decay_gauss_quad.pdf}}
    \enspace
    \subfloat[Sanity check with decaying learning rate.]{\includegraphics[width=0.24\textwidth] {Plots/PlotsKnown/decay_gauss_quad.pdf}}
    \enspace
    \subfloat[Sinusoidal noise and quadratic costs.]{\includegraphics[width=0.25\textwidth]{Plots/PlotsKnown/sin_quad_6.pdf}}
    \enspace
    \subfloat[Sinusoidal noise and $L_1$ costs.]{\includegraphics[width=0.22\textwidth] {Plots/PlotsKnown/sin_6_L1.pdf}}
    \enspace \\
    \subfloat[Random walk noise on simple LDS and quadratic costs.]{\includegraphics[width=0.25\textwidth] {Plots/PlotsKnown/random_walk_quad_6.pdf}}
    \enspace
    \subfloat[Random walk noise on simple LDS and $L_1$ costs.]{\includegraphics[width=0.23\textwidth] {Plots/PlotsKnown/physics_grw_3_L1.pdf}}
    \enspace
    \subfloat[Sinusoidal noise on complex LDS and $L_{\infty}$ cost.]{\includegraphics[width=0.23\textwidth] {Plots/PlotsKnown/semi_physics_sin_Linf.pdf}} 
    \enspace
    \subfloat[Sinusoidal noise on complex LDS and ReLU costs.]{\includegraphics[width=0.23\textwidth] {Plots/PlotsKnown/semi_physics_sin_ReLU.pdf}}
    \end{tabular}
    \caption{Known dynamics, small and large LDS setting.}
\end{figure}


==> arxiv/7.2.ExpUnknownDynamics-arxiv.tex <==

\subsection{Control with unknown dynamics}
Next, we evaluate algorithm \ref{alg3} on unknown dynamical systems. We obtain estimates $\hat{A}$ and $\hat{B}$ of the system dynamics using two different types of system identification methods, the first being the method described in algorithm \ref{alg:sys-id}, and the second being regular linear regression based on all observations up to the current time point. We then proceed with the experiments as in the previous section, with all algorithms being given $\hat{A}$ and $\hat{B}$ instead of the true $A, B$. That is, LQR produces policy $\hat{K}$ based on the solution of the algebraic Riccati equation given by $\hat{A}$ and $\hat{B}$, and both BPC and GPC start from this initial $\hat{K}$ and obtain estimates of the disturbances $\hat{w}_t$ based on the approximate dynamics. 

We run experiments with quadratic costs for the first LDS described in the known dynamics section, with scaled down dynamics matrices $A$ and $B$ such that their nuclear norm is strictly less than 1 so that the dynamical system remains stable during the identification phase. The system identification phase is repeated for each experiment and runs for $T_0 = 5000$ time steps and with initial control matrix $K$ set to 0.

\begin{figure}[H]
    \centering
    \begin{tabular}{cc}
    \subfloat[Sanity check]{\includegraphics[width=0.30\textwidth] {Plots/PlotsUnknown/sysid-regular-gauss-H3.pdf}}
    \enspace
    \subfloat[Sinusoidal noise]{\includegraphics[width=0.30\textwidth] {Plots/PlotsUnknown/sysid-regular-sin-H3.pdf}}
    \enspace
    \subfloat[Random walk noise]{\includegraphics[width=0.30\textwidth] {Plots/PlotsUnknown/sysid-regular-walk-H6.pdf}}
    \\
    \subfloat[Sanity check]{\includegraphics[width=0.30\textwidth] {Plots/PlotsUnknown/sysid-regress-gauss-H6.pdf}}
    \enspace
    \subfloat[Sinusoidal noise]{\includegraphics[width=0.30\textwidth] {Plots/PlotsUnknown/sysid-regress-sin-H3.pdf}}
    \enspace
    \subfloat[Random walk noise]{\includegraphics[width=0.30\textwidth] {Plots/PlotsUnknown/sysid-regress-walk-H3.pdf}}
    \end{tabular}
    \caption{Unknown dynamics, the top row uses the system identification method in algorithm \ref{alg:sys-id}, and the bottom row uses linear regression.}
\end{figure}
